EUFCC-CIR: a Composed Image Retrieval Dataset for GLAM Collections

The intersection of Artificial Intelligence and Digital Humanities enables researchers to explore cultural heritage collections with greater depth and scale. In this paper, we present EUFCC-CIR, a dataset designed for Composed Image Retrieval (CIR) within Galleries, Libraries, Archives, and Museums (GLAM) collections. Our dataset is built on top of the EUFCC-340K image labeling dataset and contains over 180K annotated CIR triplets. Each triplet is composed of a multi-modal query (an input image plus a short text describing the desired attribute manipulations) and a set of relevant target images. The EUFCC-CIR dataset fills an existing gap in CIR-specific resources for Digital Humanities. We demonstrate the value of the EUFCC-CIR dataset by highlighting its unique qualities in comparison to other existing CIR datasets and evaluating the performance of several zero-shot CIR baselines.

==> sota.tex <==
\section{Related Work}
\label{sec:sota}
In recent years there has been a growing interest on new models for Composed Image Retrieval (CIR), where the input query is specified in the form of an image plus some text that describes desired modifications. In this section, a general description will be presented about different models and datasets that aim to achieve Composed Image Retrieval.

Vo \etal~\cite{vo2019composing} proposes a model that makes use of a gate mechanism in order to bring closer the embedding spaces of the image plus text query and the target image. The proposed is named  TIRG, an abbreviation standing for ``Text Image Residual Gating''.


{\color{blue}
In a seminal paper for the CIR task, Vo \etal~\cite{vo2019composing} proposes a model that makes use of a gate mechanism in order to bring closer the embedding spaces of the image plus text query and the target image. The proposed is named  TIRG, an abbreviation standing for ``Text Image Residual Gating''. 
The TIRG method consists on encoding the query image $x$ using a ResNet-17 CNN, resulting in a 2D spatial feature vector $f_{img}(x) = \phi_x \in \mathbb{R}^{W X H X C}$, where W is the width, H is the height, and $C = 512$ is the number of feature channels. Then, they encode the query text using a LSTM, obtaining $f_{text}(t)=\phi_t \in \mathbb{R}^d$, where $d = 512$. In the end, the composition of these two embeddings is done using $\phi_{xt}=f_{combine}(\phi_x, \phi_t)$. In particular, $\phi_{xt}$ is implemented as a weighted sum of the gating and the residual features: $\phi^{rq}_{xt} = w_g f_{gate}(\phi_x,\phi_t) + w_r f_{res} (\phi_x,\phi_t)$, where $w_g$ and $w_r$ represent learnable weights to balance the two gates.
% i think it's wrong: This function is meant to modify (displace) the query image feature using the textual features, instead of traditional fusion of the features that creates a new feature from existing ones.

%The model is tested against three datasets: Fashion-200K \cite{han2017automatic}, MIT-States \cite{isola2015discovering} and a new synthetic dataset named CSS (standing for Color, Shape and Size). CSS is based on the CLEVR framework \cite{johnson2017clevr}, and was created because of the lack of complexity in the text modifications on the other existing CIR datasets. 
% insert information about VQA and T smth (the other gate)



TIGR outperforms several baselines for the task of CIR, including image-only (using only the image modality as query), text only (using only text as query), and other multi-modal retrieval methods in several benchmark datasets. %For the FashionIQ it produces a recall R@1 of $14.1^{\pm0.6}$, at R@10 of $42.5^{\pm0.7}$ and at R@50, $63.8^{\pm0.8}$. MIT-States scores: $R@1 = 12.2^{\pm0.4}$, $R@5 = 31.9^{\pm0.3}$ and $R@10 = 43.1^{\pm0.3}$. Lastly, running the TIRG model on the CSS produces the result of $73.7^{\pm1.0}$ for recall $R@1$.


Han \etal~\cite{han2022uigr} proposed a Unified Interactive Garment Retrieval (UIGR) method that exhibits a specialization in the domain of garment retrieval, predicated upon the consideration of two distinct contributing factors: Text-guided garment retrieval (TGR) and Visually compatible garment retrieval (VCR). In short, both methods make use of the user feedback. The TGR is focused on the changes to the piece of cloth in the image, in terms of attributes. For example, the user introduces an image with a shirt with short sleeves and asks for a shirt that has longer sleeves. Meanwhile, VCR is harnessed to prognosticate fashion compatibility, aiming to ascertain the aesthetic harmonization between two garments of distinct categories. For instance, the user would like to find the matching shoes for a certain pair of jeans. In this case, the shoes and jeans are part of different categories, whereas, in the case of TGR, it is searching only in the category of shirts. %A visual representation of the difference between these methods in seen in \autoref{fig:tgr_vcr_example}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.5\linewidth]{vcr_tgr_example.png}
%    \caption{An example of IGR (Interactive garment retrieval), which include both VCR and TGR. We can see that the user initiate the flow with a desire to change the jeans' color to gray, providing an input image of blue jeans and the prompt with the modification. The operation involves TGR, as it searches only in the category of jeans. It is then followed by a VCR operations, since the feedback suggests looking into another clothing category, to match the selected jeans. The process ends with another TGR operation, because the user wishes to modify the cardigan selected at the previous step, implying looking for a pair in the category of sweaters. Figure source: Han \etal\cite{han2022uigr}}
%    \label{fig:tgr_vcr_example}
%\end{figure}

The initial factor pertains to soliciting user feedback, which serves as a guiding mechanism in the search process. Based on it, the system chooses to follow either VCR or TGR. The proposed architecture for UIGR is shown in \autoref{fig:uigr}. This approach demonstrated superior performance compared to TIRG on the FashionIQ dataset. %To evaluate their model's performance, they separately computed R@10 and R@50 for both VCR and TGR, and then calculated the average from these four values. The results showed that TIRG scored 70.59, whereas the proposed method reached 72.07.

%\begin{figure} [H]
%\centering
%  \includegraphics[width=0.5\linewidth]{UIGR.png}
%\caption{Proposed architecture for UIGB. Two
%branches are used for separately learning two composition processes with shared image and signal encoder. A Branch classifier is used to distinguish the input of the user, based on which it will decide which branch will be used to determine the composition of the inference. Figure source: Han \etal~\cite{han2022uigr}.}
%\label{fig:uigr}
%\end{figure}


Baldrati \etal \cite{baldrati2022conditioned} proposed an approach that encompasses a dual-stage process. In the first stage they fine-tune the CLIP text encoder to adapt its embedding space to the task they want to address. In the second stage they train a Combiner network which learns to fuse the multi-modal features extracted with the CLIP image encoder and the fine-tuned CLIP text encoder. The Combiner's purpose, is to be able to move between two points in the image space using the textual information as displacement vectors in the image embedding space. This approach leads to better performance than previous methods by leveraging CLIP pre-trained encoders and a simple fine-tuning training procedure. %It exceeds the TIRG's R@50 of 90.03, by scoring a R@50 of 95.93.

%\begin{figure}[H]
%     \centering
%     \begin{subfigure}[b] {\textwidth}
%         \centering
%         \includegraphics[width=0.82\textwidth]{combiner - stage 1.png}
%         \caption{First stage of training overview. In this stage, using a contrastive loss, we fine-tune the CLIP text encoder to %adapt its embedding space to the conditioned image retrieval task}
%         \label{fig:combiner_stage_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b] {\textwidth}
%         \centering
%         \includegraphics[width=0.82\textwidth]{combiner - stage 2.png}
%         \caption{Second stage of training overview. In this stage, always using a contrastive loss, we train from scratch a Combiner network which learns to fuse the multimodal features extracted with the CLIP encoders.  }
%         \label{fig:combiner_stage_2}
%     \end{subfigure}
%     \caption{Two-stage training process of the Combiner Network. Figure source: Baldrati \etal \cite{baldrati2022conditioned}}
%     \label{fig:combiner_network_architecture}
%\end{figure}


Neculai \etal \cite{neculai2022probabilistic} investigates a more challenging scenario for composing multiple multi-modal queries in image retrieval. Given an arbitrary number of query images and (or) texts, the goal is to retrieve target images containing the semantic concepts specified in multiple multimodal queries. It is proposed a new benchmark with a comprehensive evaluation of multiple state-of-the-art multi-modal methods and propose a novel Multimodal Probabilistic Composer (MPC). Rather than fusing embeddings from different modalities through a fixed set of learnable parameters, they parameterize each input as a probabilistic embedding~\cite{chun2021probabilistic} following a multivariate Gaussian, and compose embeddings by deriving a composite multivariate Gaussian based on a probabilistic composition rule. %The overview of the model is shown in \autoref{fig:mpc_schema}.

For CIR task, in cases where the query comprises both an image and text, MPC surpasses the TIRG model in the FashionIQ dataset, %achieving a score of 9.10 relative to 4.87.
while for inputs formed of three queries (two images plus a text prompt), the difference is even more pronounced.%, achieving 4.15, in comparison to TIRG's 1.30.

%\begin{figure} [H]
%\centering
%  \includegraphics[width=\linewidth]{MPC Schema.png}
%\caption{MPC Model overview. Initially, MPC leverages two queries to simplify visual understanding, although this can be scaled to accommodate any number of input queries. The process begins with MPC acquiring knowledge from two modality-specific probabilistic embeddings. Subsequently, these two embeddings are harmonized through a probabilistic composition process, resulting in a probabilistic compositional embedding. This compositional embedding is further aligned with the probabilistic embedding of the target image "t" by minimizing a probabilistic distance metric. Figure source: Neculai \etal \cite{neculai2022probabilistic}.}
%\label{fig:mpc_schema}
%\end{figure}


Up to here all the reviewed methods are supervised models. They need training data that is specifically annotated for the CIR task. The method presented by Saito \etal \cite{saito2023pic2word} is the first zero-shot model that has attempted to do CIR. The proposed method (Pic2Word) consists of a pre-trained image-text model, CLIP (Contrastive Language Image Pretraining) \cite{radford2021learning}, which is designed to discover representations that align images with their corresponding captions while distinguishing unpaired instances. The output embeddings of two encoders (image and text) are aligned with respect to each other’s modality. Given a frozen pre-trained model, Saito~\etal \enspace train a mapping network to convert the visual embedding of the input image into a corresponding pseudo-language token. In this way they can convert a multi-modal query into a single modality (text). The network is optimized such that the pseudo token represents the visual embedding faithfully. At test time the predicted token is simply inserted into a template together with the query text and the resulting features are compared to candidate images. %The process is illustrated in \autoref{fig:pic2word_schema}.


%\begin{figure}[H]
%\centering
%  \includegraphics[width=\linewidth]{pic2word_schema.png}
%\caption{\textbf{Left}: Overview of training our Pic2Word mapping network. The mapping network, f\textsubscript{M}, is optimized to minimize the contrastive loss between the image embedding and the language embedding generated by the pseudo word token s, creating a language embedding that is compatible with the embedding generated by the frozen CLIP language encoder. \textbf{Right}: Overview of inference. The estimated token is used to fill in the given prompt sentence. Figure source: Saito \etal \cite{saito2023pic2word}.}
%\label{fig:pic2word_schema}
%\end{figure}

The mapping network in Pic2Word model is implemented as a 3 layer MLP and is trained on the Conceptual Captions dataset \cite{sharma2018conceptual}; its zero-shot capabilities are evaluated against FashionIQ \cite{wu2021fashion}, CIRR \cite{liu2021image}, ImageNet \cite{deng2009imagenet} and COCO \cite{lin2014microsoft}. Across these four datasets, Pic2Word demonstrates robust generalization in various Compositional Image Retrieval tasks. Its performance matches or surpasses several recent CIR supervised methods that necessitate labeled training data. %For example, in comparison with Baldrati's Combiner \cite{baldrati2022conditioned}, the score of the mean recall over 50 for FashionIQ \cite{wu2021fashion} dataset is 43.7 to 57.2, in favor of the Combiner \cite{baldrati2022conditioned}.


From the previous literature review we can see some open challenges in the task of CIR. The first one would be the need of large scale annotated datasets which are expensive to collect. Although the zero-shot setting proposed by Saito \etal \cite{saito2023pic2word} solves this problem, it also has some drawbacks such as the possible domain gap between pre-training and inference data or the limitation that it is encoding the whole image as a single text token, which implies an information bottleneck in complex scenes. In this research project we investigate some for this challenges and propose a new model based on the Pic2Word architecture that can handle images with more than one object.

}

%adapt the old state of the art to what we have


{\color{blue}
\subsection{Datasets}
%fer-ho més curt I mencionar algun dataset més, dels links que tinc I agafar les característiques. Això perquè quan presentem el dataset, haurem de fer un paragraf amb els trets diferencials del nostre dataset envers la resta. => db aplicat al sector GLAM, I si surt alguna cosa més
% db a incloure. fashion
% fer una taula comparativa al final dels tamanys dels datasets, number of samples, train/test

\label{sec:datasets}

The TIGR model was tested against three datasets: Fashion-200K \cite{han2017automatic}, MIT-States \cite{isola2015discovering} and a new synthetic dataset named CSS (standing for Color, Shape and Size). CSS is based on the CLEVR framework \cite{johnson2017clevr}, and was created because of the lack of complexity in the text modifications on the other existing CIR datasets. 

For the experiments conducted we are using CSS and COCO datasets. CSS is a dataset created by Vo \etal \cite{vo2019composing}, because of the need for complex text modifiers in the CIR task. Each CSS image scene is rendered with the Blender3D software by randomly sampling sets of objects. The following sets are created to describe the attributes of each objects:
\begin{itemize}
    \item Colors: cyan, yellow, green, blue, brown, gray, purple, red
    \item Shapes: rectangle, cylinder, triangle, circle 
    \item Sizes: small, large
\end{itemize}

For the modifications that can be done to an image, they created the subset \{add, remove, change object attribute\}. The ``add object'' modification allows the specification of a new object to be introduced into the scene, including its characteristics such as color, size, shape, and position. In cases where any of these attributes are unspecified, their values will be selected randomly. For instance, examples of this modification include ``add object'', ``add a red cube'', and ``add a large red cube to the middle-center position''.

Similarly, the ``remove object'' modification specifies an object within the scene for removal. All objects that match the specified attribute values will be removed. For example, one can issue commands like ``remove the yellow sphere'' or ``remove the object at the middle-center position''.

Lastly, the ``change object'' modification identifies an object to be altered, along with the desired attribute change, which can pertain to either color or size. All objects sharing the specified attribute will undergo the change. For instance, users can instruct the system with commands like ``resize the yellow sphere to a smaller size'' or ``alter the color of the object at the middle-center position to red''.

In total, a number of 32K queries are created, being split equally into a train set and a test set. These queries consists of tuples of referenced image, text prompt and the target image. Examples of these pairs are displayed in the \autoref{tab:css_examples_pairs}. 

Every image in the CSS dataset has a corresponding JSON file that describes the entire scene. Starting with the provided center pixel coordinates of every object, we obtained the bounding boxes of each shape using Segment Anything, which we further save as a new attribute to the scene JSON file. They might be of use for further experiments involving the bounding boxes.



Another dataset that we used for the experiments is the validation set of the COCO dataset. 
In Pic2Word, the evaluation of the COCO dataset consists of a query containing an image with a single object and a list of class labels that the target image should include. An example of their COCO evaluation subset is shown in \autoref{fig:original_pic2word_coco_example}. We notice that by utilizing this approach, it becomes impossible to incorporate prompts for removing or altering specific attributes of the objects in the image, or to use input image queries with more than one object. Having this in mind, we constructed a small dataset to evaluate the behavior of a CIR model with regard to this type of images, while including more natural language captions similar to what the input of a user might look like. This dataset will be further referred to as SmallCOCO-CIR. 


%In contrast to the Pic2Word evaluation approach of the COCO, where the query contains an image and a list of classes that the target image should include, in addition to the classes that already exists in the query image, we decided to pursue the creation of captions similar to what a user would write. By classes, they are referring to classes of objects that are part of COCO dataset, for example: car, cat or people. 


}























% add this and if there space missing I will put it:
We can see some open challenges in the task of CIR. The first one would be the need of large scale annotated datasets which are expensive to collect. 

CSS~\cite{vo2019composing} (standing for Color, Shape and Size) is a synthetic dataset based on the CLEVR framework \cite{johnson2017clevr}, and was created because of the lack of complexity in the text modifications on the other existing CIR datasets. CSS is a dataset created because of the need for complex text modifiers in the CIR task. Each CSS image scene is rendered with the Blender3D software by randomly sampling sets of objects. The following sets are created to describe the attributes of each objects:
\begin{itemize}
    \item Colors: cyan, yellow, green, blue, brown, gray, purple, red
    \item Shapes: rectangle, cylinder, triangle, circle 
    \item Sizes: small, large
\end{itemize}
For the modifications that can be done to an image, they created the subset \{add, remove, change object attribute\} and vary the queries based on these attributes.

\label{sec:datasets}

Another dataset is used for the experiments is the validation set of the COCO dataset. 
In Pic2Word, the evaluation of the COCO dataset consists of a query containing an image with a single object and a list of class labels that the target image should include. An example of their COCO evaluation subset is shown in \autoref{fig:original_pic2word_coco_example}. 


FashionIQ: This dataset consists of fashion images from three categories: Dress, Shirt, and Tops&Tees. It is designed for interactive image retrieval with natural sentence queries that describe modifications.

Shopping100k: This large-scale fashion dataset contains images of individual clothing items. Categories include attributes like collar, color, fabric, fit, gender, and pattern. It is particularly useful for evaluating retrieval models that need to handle a wide variety of clothing attributes and styles.

CIRCO (Composed Image Retrieval on Common Objects): Based on real-world images from the COCO 2017 unlabeled set, CIRCO is designed to address issues in existing CIR datasets by providing multiple ground truths and reducing false negatives. 

CIRR (Compose Image Retrieval on Real-life images): This dataset consists of real-life images designed to overcome issues of visual complexity and false negatives in image retrieval datasets. Images are grouped into sets of six visually similar images, and queries ensure that reference and target images belong to the same set. 


